Breaking the Computation and Communication Abstraction Barrier in Distributed Machine Learning Workloads

Recent trend towards increasing large machine learning models require both training and inference tasks to be distributed. Considering the huge cost of training these models, it is imperative to unlock optimizations in computation and communication to obtain best performance. However, current logical separation between computation and communication kernels in deep learning frameworks misses the optimization opportunities across such barrier. Breaking this abstraction with a holistic consideration can provide many optimizations to provide performance improvements in distributed workloads. Manually applying these optimizations needs modifications in underlying computation and communication libraries for each scenario, which is time consuming and error-prone. Therefore, we present CoCoNeT, with a DSL to express a program with both computation and communication. CoCoNeT contains several machine learning aware transformations to optimize a program and a compiler to generate high performance kernels. Providing both computation and communication as first class constructs allows users to work on a high-level abstraction and apply powerful optimizations, such as fusion or overlapping of communication and computation. CoCoNeT enables us to optimize data-, model-and pipeline-parallel workloads in large language models with only a few lines of code. Experiments show CoCoNeT significantly outperforms state-of-the-art distributed machine learning implementations.

==> background.tex <==
\section{NCCL Overview}
\label{sec:background:nntraining}
% \begin{figure}
%   \includegraphics[width=\columnwidth,page=2]{figures/motivation}
%   \vspace{-1.5cm}
%   \caption{A simple data-parallel example demonstrating the
%     unnecessary memory movement, redundant computation on multiple
%     GPUs, and multiple expensive GPU kernel calls. Tensors with the
%     same values on different GPUs have the same fill while colors
%     denote layers in a model.  \label{fig:motivation}}
% \end{figure}
% This section first provides an overview of the common parallelization
% strategies in ML training and inference and then discusses a simple
% example that shows how existing distributed computations leave
% performance on the table. Finally an overview of NCCL~\cite{nccl} library is provided.

% \subsection{Parallelism in Machine Learning}
% \paragraph{Data Parallel Training} Data Parallel Training~\cite{data-parallelism} distributes the training dataset 
% evenly among all GPUs and replicates the model parameters on each. Each GPU independently 
% calculates forward and backward passes based on its dataset and computes the gradients for each layer of the model.
% Followed by the backward pass, gradients across GPUs are averaged and replicated on each device. The averaged gradients
% are fed to an \emph{optimzer} such as SGD~\cite{sgd}, momentum~\cite{momentum}, Adam~\cite{adam}, LAMB~\cite{lamb} and etc.
% Adam is one of the most common optimizers used in todays training workloads such as Bert~\cite{bert}.
% % The combination of communication and then parameter update using Adam is refer to \emph{synchronous} Adam.
% % Networks such as Bert~\cite{bert} are trained using this method.
% % However, networks with large number of parameters, such as MegatronLM~\cite{megatronlm} that contains 8 Billion parameters cannot trained using this technique. 

% \paragraph{Model Parallelism}
% Model parallelism is another source of parallelism which is applied to both training and inferencing. In model parallelism,
% the parameters of a model are distributed among GPUs to reduce the memory usage and parallelize the computation of each layer of
% the model. In this parallelism, all GPUs share the same input data but each GPU is responsible for computation of part of the model.
% Model parallelism is specially important for very large models that do not fit into a single GPU's memory. Example of such parallelism
% is in MegatronLM~\cite{megatronlm} models with up-to 8 Billion parameters.

% % Data Parallel Training cannot be used if the model size is not small enough to fit into the memory of a single process. 
% % Hence, Model Parallel Training~\cite{model-parallelism} is used, where the model is split among processes, such that, each process is responsible of training of its own parameters. But the same dataset is provided to all processes. 
% % Communication among all processes reduce the trained parameters. 
% % Model Parallelism has been used in MegatronLM~\cite{megatronlm} to train transformer based models with 8 Billion parameters.

% \paragraph{Example 1.}
% Consider the following data-parallel computation inspired by the 
% BERT Python training scripts from NVIDIA:
% \begin{lstlisting}[language=Python]
%   gs = compute_gradients()
%   gs_flat = flatten(gs)
%   gs_flat_sum  = Allreduce(gs_flat)
%   gs_sum = unflatten(gs_flat_sum)
%   ws = [ws[i] - lr * gs_sum[i]
%         for i in range(len(ws))]
% \end{lstlisting}
% Figure~\ref{fig:motivation} pictorially depicts this computation on
% two GPUs.  Each GPU first computes 4 gradients from 4 layers with different 
% input data (denoted by different fill in each box).  Then, the GPUs copy those
% gradients into contiguous memory called
% \lstinline[language=Python]{gs_flat} to ensure the resulting
% \lstinline[language=Python]{Allreduce} is efficient.  At that point,
% each GPU copies memory out of the contigous buffers into the
% respective gradient locations and completes by updating the model
% parameters \lstinline[language=Python]{ws}. 
% $\Box$

% The above example points out three significant issues with such
% code. First, because Allreduce is a library abstraction which requires
% contiguous memory for a performant execution, each GPU does the \emph{unnecessary} flattening
% into contiguous and unflattening out of contigous memory.  Second, in
% data-parallel training, each GPU has a carbon-copy of the model
% parameters \lstinline[language=Python]{ws} and thus after the
% \lstinline[language=Python]{Allreduce}, any pointwise computation is
% \emph{redundant} as each GPU is replicating work of others.  And,
% lastly, if each statement in the above code maps to a single GPU
% kernel call, there are many \emph{unnecessary} high-overhead kernel
% calls, at least one for each line, that can be fused (in the limit)
% into a single one.
% %
% \tool{} addresses all of these issues with an easy to use and
% expressive language, compiler, and runtime.  The following section
% defines the syntax and semantics of our language while later
% Section~\ref{sec:functional-primitives} dicsuss the compiler and
% Section~\ref{sec:runtime} dicscues how \tool{} turns NCCL into a
% runtime execution environment that our compiler targets.

% %\aj{@Amir can you please add details about it here.} 

% % \subsection{Synchronous Adam Optimizer}
% % Adam~\cite{adam} is a widely used optimizer. 
% % Parameter update using Adam is done by first generating the gradient $g$ for all parameters $p$ in the backward pass by each process.
% % Then mean of all gradients is determined using communication collective called \allreduce.
% % Finally, parameter $p$ are updated based on the mean of gradients, momentum ($m$), velocity($v$), learning rate ($lr$), and $\beta_1$, $\beta_2$.
% % Figure~\ref{fig:FusedSGD} shows CUDA code for parameter update using synchronous Adam with \allreduce operation of NVIDIA NCCL~\cite{nccl} library. 





% %  in the following manner:
% % \begin{align*}
% % &m_{t+1} = \beta_1 \times m[t] + (1-\beta_1)*g\\
% % &v_{t+1} = \beta_1 \times v[t] + (1-\beta_1)*g^2\\
% % &m_{t+1}' = m_{t+1} \div (1 - \beta_1)\\
% % &v_{t+1}' = v_{t+1} \div (1 - \beta_2)\\
% % &p = p - lr \times m_{t+1}' \div \left(\sqrt{v_{t+1}'} + 10^{-6}\right)
% % \end{align*}

% % \begin{figure}[t]
% %   \footnotesize
% %         \begin{lstlisting}[language=C++]
% % __global__ void adamUpdate(float* p, float* g, 
% %         float* v, float* m, float lr, 
% %         float beta1, float beta2, size_t N) {
% %   i = threadIdx.x + blockDim.x*blockIdx.x;
% %   if (i < N) {
% %     m[i] = beta1*m[i] + (1-beta1)*g[i];
% %     v[i] = beta2*v[i] + (1-beta2)*g[i]*g[i];
% %     m_ = m[i]/(1-beta1);
% %     v_ = v[i]/(1-beta2);
% %     p[i] = p[i] - lr * m_/sqrt(v_ + 1e-6); }}

% % void synchronousAdam(float *p, float* g, float* v, 
% %                 float* m, float lr, float beta1, 
% %                 float beta2, size_t N){
% %   ncclAllReduce(g, g, ncclFloat, N);
% %   sgdUpdate(p, g, v, m, lr, beta1, beta2, N); }
% %         \end{lstlisting}
% %     \caption{Parameter Update using Synchronous Adam\label{fig:FusedSGD}}
% % \end{figure}

% %\subsection{NCCL Overview}
% %\label{sec:background:nccl-overview}
NVIDIA Collective Communication Library~\cite{nccl} (NCCL) is a communication library for NVIDIA GPUs.
NCCL provides communication primitive such as send and recv, and communication collectives to communicate between NVIDIA GPUs.
Moreover, these functions follows MPI standards~\cite{mpi} and terminology.
In the rest of the paper, we follow MPI terminology to represent the process ID of a distributed process as \emph{rank} and the set of all processes as \WORLD, such that, ranks ranges from $0$ to $|\WORLD|-1$.
NCCL provides five communication collectives and each takes an input buffer $b_i$ of size $N_i$ and writes to an output buffer $b_o$ of size $N_o$.
\emph{\allreduce} performs a reduction operation on $b_i$ and leaves identical copies of $b_o$ on all ranks.
\emph{\allgather} gathers all $N_i$ values of $b_i$ from all ranks to $b_o$, such that, $N_o = N_i \times |\WORLD|$.
\emph{\reducescatter} performs a reduction operation on $b_i$ and scatter the result among all ranks in $b_o$, such that, $N_o = N_i \div |\WORLD|$.
\emph{\reduce} takes a root rank $r$ and performs reduction on $b_i$ and only writes the result to $b_o$ of $r$.
\emph{\broadcast} takes a root rank $r$. It copies $N_i$ values of $b_i$ of rank $r$ and leaves identical copies in $b_o$ of all ranks.


==> fused-comm-coll.tex <==
\section{Fused Communication Collectives}
In this section, we describe bla bla bla \aj{TODO}

All communication collectives provided by NCCL can be conceptually described using a series of three primitives: (i) \texttt{SEND} that sends data from one rank to other, (ii) \texttt{RECV} that receives data from another rank, and (iii) \texttt{REDUCE} that performs reduction based on a reduction operator.
For example, in \reduce each rank first \texttt{SEND}s data, then the destination rank \texttt{RECV}s data, and finally the destination rank performs \texttt{REDUCE} on the data received.
In distributed model training, it is common that pointwise computations are performed on the data received after communication collectives, or the input to communication collectives are output of a pointwise computations.
For example, in synchronous Adam the average of all gradients distributed among different ranks is obtained using \allreduce and several pointwise computations are performed to do parameter update.
Existing techniques writes the output of communication collectives to a memory location, loads from that location and performs the computation.
Hence, this requires one store for storing the output and one load for loading the output.

However, we can remove these extra stores and loads by fusing the pointwise computations with any of the primitives, thereby passing the results of communication collectives to the computation from registers instead.
For example, 

\begin{table*}
  \small
  % \begin{subtable}{\textwidth}
    \begin{tabular}[]{|l|l|l|l|l|}\hline
      \thead{Computation with\\ Communication Collective} & Series of Primitives & Fused Communication Collective\\ \hline
      $f_2($\reduce($f_1(t)$,redOp)) & $f_1(t)\rightarrow$ SEND $\rightarrow$ RECV $\rightarrow$ $f_2$(REDUCE(redOp)) & FusedReduce(t, $f_1$, redOp, $f_2$)\\ \hline
      $f_2($\broadcast($f_1(t)$)) & $f_1(t)\rightarrow$ SEND $\rightarrow$ $f_2$(RECV) & FusedBroadcast(t, $f_1$, $f_2$)\\ \hline
      $f_2($\allreduce($f_1(t)$,redOp)) & \thead{$f_1(t)\rightarrow$SEND $\rightarrow$ RECV $\rightarrow$ $f_2$(REDUCE(redOp)) \\$\rightarrow$ SEND $\rightarrow$ RECV} & FusedAllReduce(t, $f_1$, redOp, $f_2$)\\ \hline
      $f_2($\reducescatter($f_1(t)$,redOp)) &  $f_1(t)\rightarrow$ SEND $\rightarrow$ RECV $\rightarrow$ $f_2$(REDUCE(redOp)) & FusedReduceScatter(t, $f_1$, redOp, $f_2$) \\ \hline
      $f_2($\allgather($f_1(t)$)) & $f_1(t)\rightarrow$SEND $\rightarrow$ $f_1$(RECV) & FusedAllGather(t, $f_1$, $f_2$)\\ \hline

    \end{tabular}

  \caption{Computation over Communication Collectives can be described in a series of SEND, RECV, and REDUCE primitives. We formalize these primitives into Fused Communication Collectives.}
\end{table*}



==> motivation.tex <==
\section{Motivation}


==> optimizations.tex <==
\section{Code Generation}
\label{sec:code-gen}
